Accretion and Outflow in Orion-KL Source I

We present ALMA observations of SiO, SiS, H$_2$O , NaCl, and SO line emission at ~30 to 50 mas resolution. These images map the molecular outflow and disk of Orion Source I (SrcI) on ~12 to 20 AU scales. Our observations show that the flow of material around SrcI creates a turbulent boundary layer in the outflow from SrcI which may dissipate angular momentum in the rotating molecular outflow into the surrounding medium. Additionally, the data suggests that the proper motion of SrcI may have a significant effect on the structure and evolution of SrcI and its molecular outflow. As the motion of SrcI funnels material between the disk and the outflow, some material may be entrained into the outflow and accrete onto the disk, creating shocks which excite the NaCl close to the disk surface.

==> table2.tex <==
% -------------------------------------- TABLE -----------------------------------------------
\begin{deluxetable*}{CCCC}   % capitals indicate math mode
\tabletypesize{\small}
\tablecaption{Measured sizes and flux densities for source I}
\tablecolumns{4}
\tablenum{2}
\tablehead{
%
\colhead{freq} &
%\colhead{beam} &
\colhead{deconvolved size} &
\colhead{integrated flux} \\
%
\colhead{(GHz)} &
%\colhead{(arcsec, PA)} &
\colhead{(arcsec, PA)} &
\colhead{(mJy)}
}
\startdata
%
% fit to VLA_pol/B2.cm.imcat.ave
43 &
%0.06 \times 0.04, 33\degr &
0.099 \pm 0.002 \times 0.057 \pm 0.002, -40.4\degr \pm 2.7\degr &
10 \pm 1 \\
%
% fit to OriPol2018/86GHz.mfs.I.cm
86 &
%0.04 \times 0.04, 82\degr &
0.142 \pm 0.005 \times 0.044 \pm 0.001, -38.0\degr \pm 1.0\degr &
48 \pm 5 \\
%
% fit to OriPol2018/cont/cont.mfs.cm
99 &
%0.04 \times 0.04, 47\degr &
0.151 \pm 0.005 \times 0.044 \pm 0.002, -37.8\degr \pm 1.3\degr &
58 \pm 6 \\
%
% fit to B6.ms0.mfs.cm
224 &
%0.04 \times 0.02, 66\degr &
0.197 \pm 0.003 \times 0.042 \pm 0.003, -37.3\degr \pm 0.4\degr &
256 \pm 25\\
%
% fit to X438c.cont.cm
340 &
%0.03 \times 0.01, 58\degr &
0.234 \pm 0.005 \times 0.042 \pm 0.002, -37.4\degr \pm 0.3\degr &
630 \pm 63 \\
%
\enddata\label{table2}
\end{deluxetable*}

==> table5.tex <==
% --- table of observations --- %
\begin{deluxetable*}{cccccc}
\tabletypesize{\small}
\tablecaption{SiO Lines and Masers}
\tablecolumns{6}
\tablenum{3}
\tablehead{
%
\colhead{transition} &
\colhead{freq} &
\colhead{energy} &
\colhead{maser} &
\colhead{shock speed}  &
\colhead{Alt. Refs.*} \\
%
\colhead{(v,j)} &
\colhead{(GHz)} &
\colhead{(cm$^{-1}$)} &
\colhead{(yes/no)} &
\colhead{(km/s)} &
\colhead{(Author, Year)}
}
\startdata
 (0,1-0)  &  43.423858     &  1.448464  &  yes  &   $\sim 10+$  & \cite{Hirota2020}  \\
 (0,2-1)  &  86.243442	&  2.876772  &  yes  &   $\sim 10+$  & \cite{Plambeck2009} \\
 (0,5-4)  & 217.10498  & 7.24184  &   no    &   $\sim 25+$ & \cite{Zapata2012} \\
 (0,8-7)  &  347.330631	&  11.585702  &   no  &   $\sim 25++$ & \cite{L_pez_V_zquez_2020} \\
 (0,10-9)  &	434.1195521  &  14.480670  &   no  &   $\sim 25++$ & \cite{Kim_2019}, \cite{Ginsburg2018} \\
 (0,12-11)  &	520.8782039  &  17.374627  &   no  &   $\sim 25+++$ & \cite{Hirota2017} \\
 (1,1-0)  &	43.122080  &  1.438398  &   yes  &   $\sim 25+$ & \cite{Greenhill1998}, \cite{Matthews2010} \\
 (1,2-1)  &	86.243442  &  2.876772  &   yes  &   $\sim 25+$ & \cite{Townes_1997} \\
 (2,1-0)  &	42.820587  &  1.428341  &   yes  &   $\sim 25+$ & \cite{Kim2008}, \cite{Matthews2010} \\
 (2,10-9)  &	428.087451  &  14.2794603  &   no  &   $\sim 25++$ & \cite{Kim_2019} \\
 (4,11-10)  &	464.244956  &  15.4855449  &   no  &   $\sim 25++$ & \cite{Kim_2019} \\
\enddata
\tablecomments{*For more information on masers please see \cite{Townes_1997}.}
\end{deluxetable*}

